Gramian Attention Heads are Strong yet Efficient Vision Learners

We introduce a novel architecture design that enhances expressiveness by incorporating multiple head classifiers (\ie, classification heads) instead of relying on channel expansion or additional building blocks. Our approach employs attention-based aggregation, utilizing pairwise feature similarity to enhance multiple lightweight heads with minimal resource overhead. We compute the Gramian matrices to reinforce class tokens in an attention layer for each head. This enables the heads to learn more discriminative representations, enhancing their aggregation capabilities. Furthermore, we propose a learning algorithm that encourages heads to complement each other by reducing correlation for aggregation. Our models eventually surpass state-of-the-art CNNs and ViTs regarding the accuracy-throughput trade-off on ImageNet-1K and deliver remarkable performance across various downstream tasks, such as COCO object instance segmentation, ADE20k semantic segmentation, and fine-grained visual classification datasets. The effectiveness of our framework is substantiated by practical experimental results and further underpinned by generalization error bound. We release the code publicly at: https://github.com/Lab-LVM/imagenet-models.

==> Tables/SUP-CIFAR.tex <==
\begin{table}[t]
\small
\centering
\tabcolsep=0.15cm
\begin{tabular}{l|cc|cc} 
\toprule
Network &\begin{tabular}[c]{@{}c@{}}FLOPs\\ (G) \end{tabular} & \begin{tabular}[c]{@{}c@{}}Params\\ (M) \end{tabular}  & \begin{tabular}[c]{@{}c@{}}Top-1\\ Err. (\%)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Top-5\\ Err. (\%)\end{tabular} \\ \midrule
PyramidNet-200~\cite{pyramidnet}$^\dagger$  & 4.57 & 26.92 & 14.47 & 2.97 \\
\ours  & 3.55 & 24.97 & \textbf{13.20} & \textbf{2.28} \\ 
\bottomrule
\end{tabular}
\caption{\small {\bf Experiment with PyramidNet.}
\ours\ is built upon PyramidNet-200 and trained only with CutMix to compare with the baseline$^\dagger$ in Yun \etal~\cite{cutmix} on CIFAR100. To validate the efficiency of ours, \ours\ use a smaller channel than the baseline. Note that the channel-dimension hyper-parameter \(\alpha\) in PyramidNet-200 is 240 for the baseline and 192 for \ours\ to show performance improvement even with smaller computational costs.
}
\label{tbl:pyra_cmp_CIFAR}
\end{table}

